ReinBo: Machine Learning pipeline search and configuration with Bayesian Optimization embedded Reinforcement Learning

Machine learning pipeline potentially consists of several stages of operations like data preprocessing, feature engineering and machine learning model training. Each operation has a set of hyper-parameters, which can become irrelevant for the pipeline when the operation is not selected. This gives rise to a hierarchical conditional hyper-parameter space. To optimize this mixed continuous and discrete conditional hierarchical hyper-parameter space, we propose an efficient pipeline search and configuration algorithm which combines the power of Reinforcement Learning and Bayesian Optimization. Empirical results show that our method performs favorably compared to state of the art methods like Auto-sklearn , TPOT, Tree Parzen Window, and Random Search.

==> ncommand.tex <==
\newcommand{mvspace}{\setlength\intextsep{0pt}} % reduce space for table

==> statedesign.tex <==
\section
\subsection{Reinforcement Learning Agent and Design of the state space}
We use two reinforcement learning agents in our experiment, i.e., the tabular Q learning and the Deep Q learning from the reinforcement learning package rlR. Deep Q Learning is used to facilitate future work for incorporating meta features from dataset, also, we are interested in investigating how well the functional approximator could work under our scenario.

A core technical issue is the encoding of state space.
\subsubsection{state space design with Tabular Learning}
Each state in the tabular learning is defined as a string. At beginning of episode it is initialized with $s_0 =$ ``$s$''. At a state of $s_i$, if action $a_i$ in $\mathcal{A}_{s_i}$ is taken according to current policy $\pi$, it transitions  to state $s_{i+1} = s_i.append(a_i)$, thus, the state string is always extended with actions in sequence and the transition between states is deterministic. Therefore, state $s_i$ always contains all historical information from start to $i$-th stage. For example, in the toy model we mentioned in Section 3.1 (Table 1), if we use 1 to 5 to represent available actions in each stage, then a state string of ``$s422$'' indicates a trajectory of ``SpatialSign'' - ``Kruskal'' - ``ksvm''. 
%It is remarkable that the number ``$2$'' denotes different operations in different stages because the state has already changed.

\subsubsection{state space design with DQN}
In the DQN framework, each state is encoded as a flat vector of all relevant operations. Starting from $s_0 = (0,0,0..,0)$, each element corresponds to one specific operation. In case of the toy example with 3 stages and 5 operations for each stage, it has a length of 15 (5*3). If $a_i$ is selected at state $s_i$, the corresponding element to the operation/action will change from 0 to 1, i.e. $s_{i+1}$: $s_i[a_i] = 1$. We will never be in the situation that one operation has been selected more than once because we always step in a direct and acylic way and operations in stages are totally  different. Hence, all previous information can be also tracked in this way.
